Ranking Neural Checkpoints

This paper is concerned with ranking many pre-trained deep neural networks (DNNs), called checkpoints, for the transfer learning to a downstream task. Thanks to the broad use of DNNs, we may easily collect hundreds of checkpoints from various sources. Which of them transfers the best to our downstream task of interest? Striving to answer this question thoroughly, we establish a neural checkpoint ranking benchmark (NeuCRaB) and study some intuitive ranking measures. These measures are generic, applying to the checkpoints of different output types without knowing how the checkpoints are pre-trained on which dataset. They also incur low computation cost, making them practically meaningful. Our results suggest that the linear separability of the features extracted by the checkpoints is a strong indicator of transferability. We also arrive at a new ranking measure, NLEEP, which gives rise to the best performance in the experiments.

==> robustness.tex <==
\subsection{Robustness of the checkpoints}
In addition to evaluating the final accuracy on the downstream tasks, we also test the robustness of the checkpoints against the hyper-parameters. A good checkpoint should be less sensitive to the hyper-parameters when we fine-tune on the downstream tasks. We select the top 10 
\begin{table}
\centering
%\vspace{-20pt}
\caption{Comparison results on the checkpoints of mixed supervision (Group I). Note that the average computation cost of singe forward pass on training examples to get the feature representation is 3.04E5 GFLOPS, we exclude the GFLOPS of the forward pass when we calculate the total GFLOPS.}
\label{tab:comparision_mixedsup_rob}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c}
\hline
 Method & Recall@$1$  & Rel@$1$  & Recall@$3$ & Rel@$3$  & Pearson & Kendall & GFLOPS  \\
 
%  ('0.00', '214.48', '0.00', '151.19', '33.38', '31.99')
% ('0.00', '246.33', '50.00', '149.11', '39.82', '42.60')
% ('0.00', '246.33', '25.00', '190.77', '42.09', '41.18')
% ('0.00', '303.27', '25.00', '219.35', '32.95', '26.49')
% ('0.00', '256.75', '25.00', '158.93', '43.87', '37.82')
\hline
  Linear (1 epoch)& 0.00 & \textbf{214.48} & 0.00 & \underline{151.19} & 33.38 & 31.99 &  \underline{4.95E4}\\
  Linear (5 epoch)& 0.00 & 246.33 & \textbf{50.00} & \textbf{149.11} & 39.82 & \textbf{42.60} &  4.97E4\\

 Linear (converged) & 0.00 & 246.33 & 25.00 & 190.77	& \underline{42.09}	& \underline{41.18} & 5.33E4 \\
 
  Fine-tune (1 epoch)& 0.00 & 303.27 & 25.00 & 219.35 & 32.95 & 26.49 &6.51E5 \\
  Fine-tune (5 epoch)& 0.00 & 256.75 & 25.00 & 158.93 & \textbf{43.87} & 37.82 & 4.28E6\\
\hline  

% ('0.00', '469.25', '0.00', '317.86', '-5.68', '6.32')
% ('0.00', '504.96', '0.00', '258.93', '-27.52', '-3.22')
% ('0.00', '301.79', '25.00', '155.36', '34.35', '34.42')
% ('0.00', '330.95', '0.00', '202.98', '30.11', '17.91')
MI ($\alpha$=0.01) & \multirow{2}{*}{0.00} & \multirow{2}{*}{469.25} & \multirow{2}{*}{0.00} & \multirow{2}{*}{317.86} & \multirow{2}{*}{-5.68} & \multirow{2}{*}{6.32} &\multirow{2}{*}{1.62E5} \\
 \citep{poole2019variational} & & & & & &\\
 

MI ($\alpha$=0.50)  & \multirow{1}{*}{0.00} & \multirow{1}{*}{504.96} & \multirow{1}{*}{0.00} & \multirow{1}{*}{258.93} &\multirow{1}{*}{-27.52}  & \multirow{1}{*}{-3.22} &1.62E5\\
% \citep{poole2019variational} & & & & & \\


MI w/ PCA ($\alpha$=0.01) & \multirow{1}{*}{0.00} & \multirow{1}{*}{301.79} & \multirow{1}{*}{25.00} & \multirow{1}{*}{155.36} & \multirow{1}{*}{34.35} & \multirow{1}{*}{34.42} &5.58E4\\
% \citep{poole2019variational} & & & & & \\


MI w/ PCA ($\alpha$=0.50) & \multirow{1}{*}{0.00} & \multirow{1}{*}{330.95} & \multirow{1}{*}{0.00} & \multirow{1}{*}{202.98} & \multirow{1}{*}{30.11} & \multirow{1}{*}{17.91} &5.58E4\\  
% \citep{poole2019variational} & & & & & \\
\hline
LEEP & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{{--}} & \multirow{2}{*}{{--}} & \multirow{2}{*}{--} & \multirow{2}{*}{--} & \multirow{2}{*}{--}\\ 
\citep{leep} & & & & & &\\
\hline
% ('25.00', '240.08', '25.00', '204.66', '38.19', '34.86')
$\mathcal{N}$LEEP & \textbf{25.00} & \underline{240.08} & 25.00 & 204.66 & 38.19 & 34.86 & \textbf{12.85}\\ 

\hline
\end{tabular}
}
\end{table}


\begin{table}
\centering
%\vspace{-20pt}
\caption{Comparison results on Supervised ResNet checkpoints (Group II). Note that the average computation cost of singe forward pass on training examples to get the feature representation is 3.04E5 GFLOPS, we exclude the GFLOPS of the forward pass when we calculate the total GFLOPS.}
\label{tab:comparision_sup_rob}


\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c}
\hline
  Method & Recall@$1$  & Rel@$1$  & Recall@$3$ & Rel@$3$  & Pearson & Kendall & GFLOPS  \\
% ('25.00', '490.70', '25.00', '185.57', '-5.47', '-3.34')
% ('0.00', '163.56', '25.00', '115.64', '23.62', '22.97')
% ('0.00', '280.10', '50.00', '108.21', '35.48', '24.45')
% ('25.00', '154.41', '25.00', '148.97', '-1.09', '-2.98')
% ('25.00', '265.52', '25.00', '115.64', '30.07', '16.45')

\hline
  Linear (1 epoch) & 25.00 & 490.70 & 25.00 & 185.57 & -5.47 & -3.34 &4.95E4\\
  Linear (5 epochs) & 0.00 & 163.56 & 25.00 & \underline{115.64} & 23.62 & 22.97 & 4.97E4\\
  
  Linear (converged) &0.00 & 280.10 &\textbf{50.00}	& \textbf{108.21}	& \textbf{35.48}	& \textbf{24.45} & 5.33E4\\
  
  Fine-tune (1 epoch) & 25.00 & 154.41 & 25.00 & 148.97 & -1.09 & -2.98 &6.51E5\\
  Fine-tune (5 epochs) & 25.00 & 265.52 & { 25.00} & { \underline{115.64}} & 30.07 & 16.45 &4.28E6\\
   
%  ('0.00', '335.33', '25.00', '127.18', '-0.68', '-8.85')
% ('0.00', '645.72', '25.00', '245.24', '-10.95', '-15.72')
% ('25.00', '158.87', '25.00', '142.72', '10.49', '5.74')
% ('0.00', '197.34', '0.00', '154.74', '21.50', '12.67')
\hline
MI ($\alpha$=0.01) & \multirow{2}{*}{0.00} & \multirow{2}{*}{335.33} & \multirow{2}{*}{25.00} & \multirow{2}{*}{127.18} & \multirow{2}{*}{-0.68} & \multirow{2}{*}{-8.85} & \multirow{2}{*}{1.62E5}\\
 \citep{poole2019variational} & & & & & &\\
 

MI ($\alpha$=0.50)  & \multirow{1}{*}{0.00} & \multirow{1}{*}{645.72} & \multirow{1}{*}{25.00} & \multirow{1}{*}{245.24} & \multirow{1}{*}{-10.95} &  \multirow{1}{*}{-15.72} & \multirow{1}{*}{1.62E5}\\
%\citep{poole2019variational} & & & & & \\


MI w/ PCA ($\alpha$=0.01) & \multirow{1}{*}{25.00} & \multirow{1}{*}{158.87} & \multirow{1}{*}{25.00} & \multirow{1}{*}{142.72} & \multirow{1}{*}{10.49} & \multirow{1}{*}{5.74} &  \multirow{1}{*}{5.58E4}\\
%\citep{poole2019variational} & & & & & \\


MI w/ PCA ($\alpha$=0.50)  & \multirow{1}{*}{0.00} & \multirow{1}{*}{197.34} & \multirow{1}{*}{0.00} & \multirow{1}{*}{154.74} & \multirow{1}{*}{21.50} & \multirow{1}{*}{12.67} & \multirow{1}{*}{5.58E4} \\  
%\citep{poole2019variational} & & & & & \\

% ('0.00', '136.25', '25.00', '123.39', '26.04', '21.69')

\hline
LEEP & \multirow{2}{*}{0.00} & \multirow{2}{*}{\textbf{136.25}} & \multirow{2}{*}{25.00} & \multirow{2}{*}{123.39} & \multirow{2}{*}{26.04} & \multirow{2}{*}{21.69} & \multirow{2}{*}{\underline{378.31}}\\ 
\citep{leep} & & & & & &\\

% ('0.00', '152.32', '50.00', '108.21', '42.29', '25.07')
\hline
$\mathcal{N}$LEEP & 0.00 & \underline{152.32} & \textbf{50.00} & \textbf{108.21} & \underline{42.29} & \underline{25.07} & \textbf{12.95}\\ 
\hline
%  \textit{Linear-End} &\textit{75.00} & \textit{99.95} &\textit{100.00}	& \textit{100.00}	& \textit{79.30}	& \textit{68.60} & \textit{3.575E5}\\
% \hline
\end{tabular}
}
\end{table}



\begin{table}
\centering
%\vspace{-20pt}
\caption{Comparison results on the checkpoints of heterogeneous architectures (Group III). Note that the average computation cost of singe forward pass on training examples is 2.73E5 GFLOPS to get the feature representation, we exclude the GFLOPS of the forward pass when we calculate the total GFLOPS.}
\label{tab:comparision_arch_rob}

\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|c|c}
\hline
 Method & Recall@$1$  & Rel@$1$  & Recall@$3$ & Rel@$3$  & Pearson & Kendall & GFLOPS  \\


% ('0.00', '332.57', '25.00', '219.21', '21.97', '12.39')
% ('0.00', '251.32', '25.00', '178.59', '31.09', '26.73')
% ('0.00', '255.71', '25.00', '184.84', '43.10', '17.76')
% ('25.00', '215.05', '50.00', '166.09', '32.09', '29.71')
% ('0.00', '261.27', '25.00', '172.34', '35.48', '33.11')

\hline
  Linear (1 epoch)& 0.00 & 332.57 & 25.00 & 219.21 & 21.97 & 12.39 &  3.37E4\\
  Linear (5 epoch)& 0.00 & 251.32 & 25.00 & 178.59 & 31.09 & 26.73 &  3.38E4\\

 Linear (converged) &0.00 & 255.71 &25.00	& 188.84	& \textbf{43.10}	&17.76 & 3.62E4\\
  Fine-tune (1 epoch)&  \textbf{25.00} & \textbf{215.05} & \textbf{50.00} & \underline{166.09} & 32.09 & 29.71 &4.43E5 \\
  Fine-tune (5 epoch)& 0.00 & 261.27 & 25.00 & 172.34 & 35.48 & \underline{33.11} & 2.91E6\\
\hline  

% ('25.00', '246.64', '25.00', '144.21', '35.13', '37.85')
% ('0.00', '236.61', '25.00', '185.07', '13.50', '20.16')
% ('0.00', '253.16', '25.00', '203.82', '23.75', '8.28')
% ('0.00', '337.72', '25.00', '185.07', '25.19', '10.93')
MI ($\alpha$=0.01) & \multirow{2}{*}{\textbf{25.00}} & \multirow{2}{*}{246.64} & \multirow{2}{*}{25.00} & \multirow{2}{*}{\textbf{144.21}} & \multirow{2}{*}{35.13} & \multirow{2}{*}{\textbf{37.85}} &\multirow{2}{*}{1.30E5} \\
 \citep{poole2019variational} & & & & & &\\

MI ($\alpha$=0.50)  & \multirow{1}{*}{0.00} & \multirow{1}{*}{\underline{236.61}} & \multirow{1}{*}{25.00} & \multirow{1}{*}{185.07} &\multirow{1}{*}{13.50}  & \multirow{1}{*}{20.16} &1.30E5\\
% \citep{poole2019variational} & & & & & \\

MI w/ PCA ($\alpha$=0.01) & \multirow{1}{*}{0.00} & \multirow{1}{*}{253.16} & \multirow{1}{*}{25.00} & \multirow{1}{*}{203.82} & \multirow{1}{*}{23.75} & \multirow{1}{*}{{8.28}} &5.56E4\\
% \citep{poole2019variational} & & & & & \\

MI w/ PCA ($\alpha$=0.50) & \multirow{1}{*}{0.00} & \multirow{1}{*}{337.72} & \multirow{1}{*}{25.00} & \multirow{1}{*}{185.07} & \multirow{1}{*}{25.19} & \multirow{1}{*}{10.93} &5.56E4\\  
% \citep{poole2019variational} & & & & & \\

% ('0.00', '771.45', '25.00', '239.16', '12.43', '-5.92')
\hline
LEEP & \multirow{2}{*}{0.00} & \multirow{2}{*}{771.45} & \multirow{2}{*}{25.00} & \multirow{2}{*}{239.16} & \multirow{2}{*}{12.43} & \multirow{2}{*}{-5.92} & \multirow{2}{*}{\underline{247.56}}\\ 
\citep{leep} & & & & & &\\

% ('0.00', '596.45', '0.00', '215.43', '36.48', '16.66')
\hline
$\mathcal{N}$LEEP & 0.00 &596.45 & 0.00 & 215.43 & \underline{36.48} & 16.66 & \textbf{12.68}\\ 

\hline
\end{tabular}
}
\end{table}
